Adaptive Learning of Aggregate Analytics under Dynamic Workloads

Large organizations have seamlessly incorporated data-driven decision making in their operations. However, as data volumes increase, expensive big data infrastructures are called to rescue. In this setting, analytics tasks become very costly in terms of query response time, resource consumption, and money in cloud deployments, especially when base data are stored across geographically distributed data centers. Therefore, we introduce an adaptive Machine Learning mechanism which is light-weight, stored client-side, can estimate the answers of a variety of aggregate queries and can avoid the big data backend. The estimations are performed in milliseconds are inexpensive and accurate as the mechanism learns from past analytical-query patterns. However, as analytic queries are ad-hoc and analysts' interests change over time we develop solutions that can swiftly and accurately detect such changes and adapt to new query patterns. The capabilities of our approach are demonstrated using extensive evaluation with real and synthetic datasets.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

==> addendum.tex <==
\section{Appendix}
\textit{Code will be made available to github with automated suite of experiments to reproduce results upon publication due to double-blind constraint.}
\subsection{Implementation \& Experimental Environment}
To implement our algorithms we used \texttt{scikit-learn} , \texttt{XGBoost}\cite{chen2016xgboost} and an implementation of the \texttt{Growing-Networks} algorithm \cite{marsland2002self}. We performed our experiments on a desktop machine with a Intel(R) Core(TM) i7-6700 CPU @ 3.40GHz and 16GB RAM. For the real datasets, the GrowingNetworks algorithm was used for clustering mainly because of its invariance to selecting a pre-defined number of clusters and it's ability to naturally grow (as required by our adaptability mechanisms). XGBoost was used as the supervised learning algorithm because of its superior accuracy to other algorithms we tested and shown as part of our evaluation.

\subsection{Real Datasets \& Workloads}
\textbf{Crimes:} 
For constructing the workload over the \textbf{Crimes} dataset we initially sampled 10K points and obtained the mean and standard deviation for the attributes \textit{X\_Coordinate},\textit{Y\_Coordinate}. By setting the obtained statistics as parameters for a multivariate normal distribution we generated a number of \textit{Cluster} points ($=5$). Centered on each one of those cluster points we constructed multivariate normal distributions with a fraction ($=0.01$) of the original standard deviation. Based on this we generated a number of points ($=10K$) for around each cluster point. Based on those points we constructed queries covering a random range across both the \textit{X/Y Coordinates}. For each point a fraction of the original std was used to construct ranges : $\text{x\_range} = \frac{\text{x\_std}}{2}\text{rand(0,1)}$, where \textit{x\_std} is the original standard deviation, same approach was followed for the \textit{y\_range}. The queries filtered the complete dataset based on (where pt is the point) :
\begin{multline}
\alpha_{X\_Coordinate} \geq \text{pt}-\text{x\_range} \land \alpha_{X\_Coordinate} \leq \text{pt}+\text{x\_range}\\
\land \alpha_{Y\_Coordinate} \geq \text{pt}-\text{y\_range} \land \alpha_{y\_Coordinate} \leq \text{pt}+\text{y\_range}
\end{multline}
On the filtered dataset generated by each query with varying cardinality we extracted basic statistics like \texttt{COUNT, AVG, SUM} on attributes that would make sense (\textit{Beat} - avg, \textit{Arrest} - sum). 

\textbf{Sensors}: 
For Sensors we obtained the mean and standard deviation of the temporal dimension after encoding it and normalizing it. The min/max statistics were also obtained. We then generated a number of queries ($=50K$) with range equal to a fraction of the complete distance between the max/min ($0.2\times(\text{max}-\text{min})$. The center of the queries was randomly generated by a normal distribution with parameters equal to the obtained mean and half original standard deviation. The same processes as in Crimes was used to filter the complete dataset and extract statistics on attributes that made sense (\textit{Temperature}-avg, \textit{Light}-sum).

\subsection{Synthetic Data Generation}
Specifically, we generated datasets with varying dimensionality $[10, 20, 50, 100]$ to simulate data with large number of columns. Each column contains numbers generated from a uniform distribution $\mathcal{U}[0, 10^{6}]$, therefore each point is $\mathbf{x} \in [0, 10^{6}]^d$ where $d \in [10, 20, 50, 100]$. We then generated a number of query workloads with a varying number of selected columns to be restricted by predicates $p \in [2, 5, 10]$ (Increasing predicates even further resulted in no tuples returned) according to the dimensionality of each of the synthetic datasets. For instance, for a dataset with $d=10$ the resulting workloads were two, with the selected columns being $(2, 10)$. Each query point for those two datasets is then $\mathbf{q} \in [0, 10^{6}]^{2p}$. The specification and the number of query workloads can be identified from Table \ref{tab:synth-workloads}.
\begin{table}[htbp]
\caption{Synthetic Datasets and Workloads}
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
& \multicolumn{4}{c|}{\textbf{Columns} ($d$)} \\ \hline
\textbf{Predicates }($p$) & $10$ & $20$ & $50$ & $100$ \\ \hline
$2$ & \checkmark & \checkmark  & \checkmark & \checkmark \\ \hline
$5$ & \checkmark & \checkmark  & \checkmark & \checkmark \\ \hline
$10$ &  & \checkmark  & \checkmark & \checkmark \\ \hline
\end{tabular}
\label{tab:synth-workloads}
\end{table}

We also describe the query generation process in Algorithm \ref{alg:query-gen}. We first set the number of queries $N$ and number of predicates and columns in our datasets $\mathcal{D}$, $\mathcal{P}$. The retrieved range size $r$ is obtained by a Normal distribution $\mathcal{N}(\text{sel}\cdot10^6, 0.01\cdot10^6)$ with the mean being a fraction of the complete range defined by selectivity ration $sel=0.5$ to ensure enough tuples are returned as with an increasing number of predicates less tuples are returned. We then loop through over the parameters issued and generated queries using the provided algorithms. Where the $random$ function returns a random vector of size $p$ over the given range, and $randomBit$ generates a random bitmask for the selection of columns taking part in the query. Then the lower-bound and upper-bound for the given predicates is set and we execute the query over the restricted space given by the bounds over the selected columns by $b$ using dataset $d$.

\begin{algorithm}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
 \caption{Generating Queries}
 \label{alg:query-gen}
 \Input{$N$, number of queries}
 \Input{$\mathcal{D} = [10, 20, 50, 100]$, number of columns in datasets}
 \Input{$\mathcal{P}= [2, 5, 10]$, number of predicates (selected columns)}
 \Input{$r$, range size retrieved from histogram to ensure similar selectivities}
 \For {$d\in \mathcal{D}$}{
 	\For {$p \in \mathcal{P}$}{
    	\For {$i= 1 \textbf{ to } N$}{
        	$\mathbf{z} \gets random(\mathcal{N}(10^6, 100), p)$ \;
            $\mathbf{b} \gets randomBit([0, d], p)$ \; 
            $\mathbf{lb} \gets \mathbf{z}-\frac{r}{2}$ \;
            $\mathbf{ub} \gets \mathbf{z}+\frac{r}{2}$ \;
            $\mathbf{q}_i^{(m)} \gets [\mathbf{lb}, \mathbf{ub}]$\;
            $y_i \gets executeAggregates(\mathbf{q}_i^{(m)}, d)$ \;
            $\mathbf{q}_i \gets (\mathbf{q}_i^{(m)},y)$ \;
            $\mathcal{W}_{d,p} \cup \{\mathbf{q}_i\}$\;
        }
    }
 }
 \Output{Resulting workloads $\mathbf{W} = (\mathcal{W}_{10,2}, \ldots, \mathcal{W}_{d,p}), \forall d\in \mathcal{D}, \forall p\in \mathcal{P}$}
\end{algorithm}



\subsection{Proofs of Theorems}
\subsubsection{Proof of Theorem 4.1}
\begin{proof}
Let the query $\mathbf{q}$ being projected to its closest representative $\mathbf{w}_{K+1}$, which is not yet converged and let its second closest be the converged $\mathbf{w}_{k}$. The representative  $\mathbf{w}_{k}$ corresponds to the mean vector of those queries belonging in the cluster $\mathcal{C}_{k}$. In order to the query $\mathbf{q}$ to be forwarded to the CS for execution it means that the $\mathbf{w}_{k}$ should not be the mean vector for the incoming query $\mathbf{q}$. This is indicated if the distance $\lVert \mathbf{q} - \mathbf{w}_{k} \rVert_{2}$ is greater than a proportion of the norm of the variance $\sigma$ of the cluster $\mathcal{C}_{k}$ by a factor $\lambda > 1$. Hence, the query is sent from the AD to the CS if at least this distance is greater than $\lambda \sigma$, which is stochasitcally bounded by the factor $1/\lambda^{2}$ based on Chebyshev's inequality $P(\lVert \mathbf{q}-\mathbf{w}_{k} \rVert_{2}) \geq \lambda \sigma \leq \frac{1}{\lambda^{2}}$.
\end{proof}    

\subsubsection{Proof of Theorem 4.2}
\begin{proof}
Each dimension $i$ of the median vector $\mathbf{m}$ of the 
queries $\mathbf{q}$ in a sub-space satisfies: 
$P(q_{i} \geq m_{i}) = P(q_{i} \leq m_{i}) = \frac{1}{2}$. 
Suppose that the new representative $\mathbf{w}_{K+1}$ has 
reached equilibrium, i.e., $\Delta \mathbf{w}_{K+1} = \mathbf{0}$ holds with probability 1.
By taking the expectations of both sides 
of the update rule $\mathbb{E}[\Delta \mathbf{w}_{K+1}] = \alpha \mathbb{E}[sgn(\mathbf{q}-\mathbf{w}_{K+1})] = \mathbf{0}$ and focusing on each dimension $i$, we obtain that: $\int sgn(q_{i}-w_{K+1,i})p(q_{i})dq_{i} = P(q_{i} \geq w_{K+1,i})\int p(q_{i})dq_{i} - P(q_{i} < w_{K+1,i})\int p(q_{i})dq_{i} = 2P(q_{i} \geq w_{K+1,i}) - 1$. Since $\mathbb{E}[\Delta w_{K+1,i}]=0$ is constant, then $P(q_{i} \geq w_{K+1,i}) =  \frac{1}{2}$, which denotes that $w_{K+1,i}$ converges to the median of $q_{i}$, $\forall i$.
\end{proof}    

\subsubsection{Proof of Theorem 4.3}
\begin{proof}
Consider that at a certain time instance, there are $n-1$ affiliate ADs which enter in their buffering mode with entry probability $\beta$. Then, the
probability of existing at least one affiliate of an AD in the CS in the buffering mode is $1-(1-\beta)^{n-1}$. Given that a query is forwarded with upper probability $O(\frac{1}{\lambda^{2}})$ for those ADs being in the buffering mode, then, the expected number of queries being executed in the CS from an AD and its affiliates within any arbitrary time interval $T$ is $T(\frac{1}{\lambda^{2}})(1 + 1-(1-\beta)^{n-1})$.
\end{proof}




==> system_architecture.tex <==
\section{System Architecture}

\begin{figure*}[!htbp]
\begin{center}
\includegraphics[width=0.8\textwidth]{figures/FotisEdge.pdf}
\caption{Analytics using ML models in a distributed setting}
\label{fig:federated-architecture}
\end{center}
\end{figure*}


\begin{figure*}[!htbp]
\begin{center}
\includegraphics[height=5cm,width=14.0cm]{sys_arch}
\caption{System architecture : Showing how our system monitors queries and then trains models that can be sent to an analyst's local machine thus freeing up resources and cutting-down costs from any cloud systems. }
\label{fig:system-architecture}
\end{center}
\end{figure*}
Our proposed system architecture is visible at Figure \ref{fig:system-architecture}. Our system sits between cloud-based data stores and/or \textit{Sampling}-based AQP engines, monitoring queries and their associated results. An analyst issues such queries using one of many available Business Intelligence (BI) tools or by programmatic-access using engines such as Spark/MapReduce/HBase etc. Our system is made up of two large modules,\textit{Partitioner} and \textit{Learner}, each responsible for different tasks as described below. The modules main job is to produce \textit{Local Models} with minimal storage costs, that can be stored in an analyst's machine and offer efficient computations for any aggregate queries the analyst may have.

\subsection{Partitioner}
The \textit{Partitioner} module is responsible for monitoring and clustering queries with respect to their parameter values as specified by the meta-vector. Queries that are clustered together denote the interests of a given analyst. If we train different ML models for those clusters of queries, we can have a separate model according to an analyst's interest that is in turn more \textit{accurate} and more lightweight.  Hence, our aim is to provide high-accuracy ML models that are better equipped to answer queries of a given analyst than if a \textit{global} model was trained on \textit{all} queries. This is in-line with an ML strategy called \textit{Mixture-of-Experts}\cite{masoudnia2014mixture}, in which multiple models are trained to handle different parts of a problem. Thus, by monitoring the queries passed to an underlying data-engine the result of a partitioner are clusters of queries pictured as 2-d color-coded (denoting association to a different cluster) points in Figure \ref{fig:system-architecture}.

\subsection{Learner}
The \textit{Learner} module is where optimization and training of ML models takes place. From our experiments we gathered that some aggregates hold properties in which different ML models are better equipped to handle. For instance, the \texttt{COUNT} operator has a monotonically-increasing behavior for ever increasing parameter-values in range queries. Thus, linear models like MARS \cite{friedman1991multivariate}, GLMs \cite{nelder2004generalized} are well equipped to handle such cases. However, other operators such as \texttt{AVG} are non-linear thus different models should be applied. This module's task is, given a cluster of queries, a sub-module called \textit{Optimizer} first runs a number of tests and applies a number of heuristics (described later) that determines which model should be used. The \textit{Trainer} is then responsible for training the specified model on the given cluster of queries. The trained model is then a lightweight module that can be easily transfered and stored on the analyst's machine who can use it to quickly obtain estimations for a number of aggregate queries.

\subsection{Local Model}
The \textit{Local Model} (shown with a $f$ in Figure \ref{fig:system-architecture}) module is essentially a light-weight component which exposes an API to the user with a single call function. Given the query's parameter-values the API returns an estimation of the result of the given query. The component can be loaded in memory as it is extremely small and thus be at the disposal of the user at any time without having to wait fetching data from disks or experiencing network latency from responses coming from distant data-centers. For any given user a number of Local Models can be transferred to her local machine with respect to the queries she has posed so far. So, given the parameter-values of the issued queries, and the aggregates she used so far the appropriate models are returned. These ensure that the answers will be highly accurate as the models have learned to generalize well over the queried-space she was using so far.


